State Estimation of Continuous-time Dynamical Systems with Uncertain Inputs with Bounded Variation: Entropy, Bit Rates, and Relation with Switched Systems

We extend the notion of estimation entropy of autonomous dynamical systems proposed by Liberzon and Mitra [1] to nonlinear dynamical systems with uncertain inputs with bounded variation. We call this new notion the {$\epsilon$}-estimation entropy of the system and show that it lower bounds the bit rate needed for state estimation. {$\epsilon$}-estimation entropy represents the exponential rate of the increase of the minimal number of functions that are adequate for {$\epsilon$}- approximating any trajectory of the system. We show that alternative entropy definitions using spanning or separating trajectories bound ours from both sides. On the other hand, we show that other commonly used definitions of entropy, for example the ones in [1], diverge to infinity. Thus, they are potentially not suitable for systems with uncertain inputs. We derive an upper bound on {$\epsilon$}-estimation entropy and estimation bit rates, and evaluate it for two examples. We present a state estimation algorithm that constructs a function that approximates a given trajectory up to an {$\epsilon$} error, given time-sampled and quantized measurements of state and input. We investigate the relation between {$\epsilon$}-estimation entropy and a previous notion for switched nonlinear systems and derive a new upper bound for the latter, showing the generality of our results on systems with uncertain inputs.

==> SwitchedSystems.tex <==
\section{Relation between the estimation entropy of Switched Systems and Slowly varying dynamical systems}
\label{sec:switched_systems}
Consider a switched nonlinear system 
\begin{align}
\label{sys:switched_system}
\dot{x}(t) = f_{\sigma(t)}(x(t)),
\end{align}
where $\sigma : \nnreals \rightarrow [N] \in \Sigma(T_d)$, is a switching signal with minimum dwell time $T_d > 0$, $\{f_p : \mathbb{R}^n \rightarrow \R^n \}_{p \in [N]}$, is a finite set of Lipschitz continuous functions with constants $L_p$'s, $x(t) \in \mathbb{R}^n$ and $x(0) \in K$, a compact initial set of states in $\mathbb{R}^n$. 
%
We can model the switched system~(\ref{sys:switched_system}) as an instance of the system with inputs~(\ref{sys:noise}).
Moreover, we can represent the minimum dwell time constraint as a constraint on the variation of the input signal by setting appropriate values for $\mu$ and $\eta$ in Definition~\ref{def:inputset} as we will show later.
% 
First, we fix a constant $u_{max}>0$ and define $U$ to be the $N$-dimensional box $[- u_{max}, u_{max}]$. Then, we map the $p^{\mathit{th}}$ mode to the $N$-dimensional vector with the $p^{\mathit{th}}$ component being $u_{\mathit{max}}$ and the rest being zeros.  We call that map $g: [N] \rightarrow U$. 
Now, we consider the mapped switching signal as the input one, i.e. it will be $\dot{x}(t) = f(x(t), g(\sigma(t)))$. In that case, $\|f(x,g(p)) - f(x',g(p))\| \leq L_p \|x - x'\| \leq L_x \|x - x'\|$, for all $x \in \mathbb{R}^n$ and $p \in [N]$, where $L_x = \max_{p \in [N]}L_p$.
% and $\delta_u = \floor{\frac{u_{max}}{N}}$. Then, we map the $N$ modes to the grid points of $grid(U, \delta_u)$. We call that map $g: [N] \rightarrow grid(U, \delta_u)$. Now, we consider the map of the switching signal as the input one, i.e. it will be $\dot{x}(t) = f(x(t), g(\sigma(t)))$. In that case, $\|f(x,g(p)) - f(x',g(p))\| \leq L_p \|x - x'\| \leq L_x \|x - x'\|$, for all $x \in \mathbb{R}^n$ and $p \in [N]$, where $L_x = \max_{p \in [N]}L_p$. for all $u \in U$, where $u_1$ and $u_2$ are the largest and smallest grid points smaller and bigger than $u$, respectively.
Then, we define 
\begin{equation}
\label{eq:switched_as_inputs}
f(x,u) := 
\begin{cases}
f_p(x), &\text{if } u = g(p), \text{ for } p \in [N], \\
0, &\text{otherwise.}
\end{cases}
\end{equation} 

Now, to compute the Lipschitz constant $L_u$ of $f$ with respect to inputs in (\ref{eq:switched_as_inputs}), we make the same assumption as in Section 2.1 of \cite{sibai-mitra-2017} that 
\begin{align}
\dist(t) := \max_{p \neq p' \in [N]}& \sup_{x \in Reach(\Sigma, K)} \nonumber \\
&\int_{0}^{t} \| f(\xi_{x,p}(s),g(p)) - f(\xi_{x,p'}(s),g(p')) \| ds
\end{align}
 is finite, we get that $\| f(x,g(p)) - f(x,g(p')) \| \leq \inf_{t > 0} d(t)/t$, for any $t > 0$, and $x \in Reach(\Sigma, K) := \{\xi_{x_0,g(\sigma)}(t)\ |\ x_0 \in K, \sigma \in \Sigma(T_d), t \geq 0\}$, the reach set of system~(\ref{sys:switched_system}), and modes $p$ and $p' \in [N]$.
 
 Since we are modeling the switched system (\ref{sys:switched_system}) as a system with inputs to get an upper bound on its entropy, we only want to bound the sensitivity of system (\ref{eq:switched_as_inputs}) with respect to inputs that correspond to switching signals in $\Sigma(T_d)$. 
 %We abuse notation and denote the map of a switching signal $\sigma \in \Sigma(T_d)$ to an input signal in $U$ by $g(\sigma)$.
 
 %Specifically, we consider the set of input signals $\mathcal{U}_s \subset \mathcal{U}$ that correspond to switching signals, i.e. for any $u \in \mathcal{U}_s$ and $t \geq 0$ there exists $p \in [N]$ s.t. $u(t) = g(p)$. 
 
 %Consider the set of pairs of input signals of the form $u,u' \in \mathcal{U}_s$ such that there exists $t_u \geq 0$ s.t. $u(t) = u'(t)$ for all $t \geq t_u$.
 Then, we define
 \begin{align*}
 \hat{L}_u :=  \max_{p \neq p' \in [N]}& \sup_{x \in Reach(\Sigma, K)}  \frac{\|f(x,g(p)) - f(x,g(p'))\|_\infty}{\|g(p)-g(p')\|_\infty}.
 %\\ &=\max\{\max_{x \in Reach(K,\mathcal{U}), u \neq u' \in U} \frac{\|f(x,u) - f(x,u')\|_\infty}{\|u-u'\|_\infty} \}
 \end{align*}
Hence, $\hat{L}_u = \liminf_{t \rightarrow 0^+} \frac{d(t)}{t u_{\mathit{max}}}$, for any $t > 0$. This $\hat{L}_u$ would not be the Lipschitz constant of $f$ in system~(\ref{eq:switched_as_inputs}) with respect to any input, but only to inputs corresponding to switching signals in $\Sigma(T_d)$. 

Let $\mathcal{U}_s(\mu,\eta,u_{\mathit{max}})$ be the set of input signals of the form: $u \in \mathcal{U}(\mu,\eta,u_{\mathit{max}})$ satisfying for every $t \geq 0$ there exists $p \in [N]$ such that $u(t) = g(p)$.
 
If we know that the minimum dwell time of the system is $T_d > 0$,  then we can compute the corresponding input variation parameters $\mu$ and $\eta$ in (\ref{variationbound}) that restricts any $u \in \mathcal{U}_s$ to have a dwell time of $T_d$.

\begin{Lemma}
	\label{lm:s_sig_to_i_sig}
Fix any $u_{\mathit{max}} > 0$ and let $\mu=\frac{u_{\mathit{max}}}{T_d}$ and $\eta = 0$. Then, any input signal $u \in \mathcal{U}_s(\mu,\eta,u_{\mathit{max}})$ has a minimum dwell time $T_d$.
\end{Lemma}
\begin{proof}
If $u \in \mathcal{U}(\mu,\eta,u_{\mathit{max}})$, then for all $t,\tau \geq 0$, $\|u(t) - u(t+\tau)\| \leq \mu \tau + \eta = \frac{u_{\mathit{max}}}{T_d} \tau$.  Hence, $u$ cannot change values in a duration shorter than $T_d$.
\end{proof}

 %Since it is allowed to switch from any mode in $[N]$ to any other mode.
 Such a restriction on the variation of the input signal would allow input signals that does not correspond to switching signals between the $[N]$ modes. Hence, it is conservative in this sense. 
 
 We first use Corollary~(\ref{cor:better_nonlinear_upperbound}) to get an upper bound on the entropy of system~(\ref{sys:switched_system}). We choose $\delta_u = u_{max}/2$. However, instead of choosing the $\ceil{\frac{u_{max}}{\delta_u}}^m = 2^m = 2^N$ points in the grid $C_u$ at line~\ref{Cu_definition} in Algorithm~\ref{fig:approxFunct} to be equidistant, we choose them to have a value of $u_{max}$ or zero at any coordinate. Moreover, instead of quantizing to the nearest point in $\mathit{quantize}$ function in line~\ref{quantU} of Algorithm~\ref{fig:approxFunct}, each coordinate of the input is mapped to $u_{max}$ if it is equal to $u_{max}$ and mapped to zero, otherwise. This way of quantization ensures that the quantized version of an input signal corresponding to a switching signal is the same signal. Since at any time an input signal does not correspond to a switching one the dynamics are zero, quantizing coordinates to zero if they are not equal to $u_{max}$ would not change the dynamics. Hence, this method of quantization preserves the correctness of Lemma~\ref{lm:proveApproxFunc}. In fact, $\delta_u$ in (\ref{eq:approxFunction_i}) can be replaced by zero and the upper bound can still correct.
 
 Since we know the Lipschitz constants $L_x$ and $\hat{L}_u$, we can use Proposition~(\ref{prop:computingMxMu}) to get $M_x$ and $M_u$. Moreover, we set $\mu$ to $\frac{u_{max}}{T_d}$ and $\eta$ to zero as in Lemma~\ref{lm:s_sig_to_i_sig}. We fix  $k=1/4$. By fixing these parameters, we get $\nu_1 = \frac{9}{2T_d}(\frac{\eps}{e M_u u_{max}})^2$. Hence, by Corollary~\ref{cor:better_nonlinear_upperbound}, if $\nu_1 \leq 1$,  the entropy $h\est(\eps,K)$ of system~(\ref{sys:switched_system}) is upper bounded by: $\frac{2n M_x}{\ln 2} +$

 \begin{equation}
 \label{eq:input_switched_bound}
 \frac{1}{ \min\big\{T_d \frac{\nu_1}{3}(1 - \frac{\nu_1}{3}),\frac{1}{M_x}\big\}}\big(n\log (1.5) +  N\log 2\big).
 \end{equation}
 
 On the other hand, we can use the bound in \cite{sibai-mitra-2017} on the entropy of system (\ref{sys:switched_system}). The definition of approximating function in \cite{sibai-mitra-2017} requires the distance between the trajectory and the function to be upper bounded by $\eps$ for a duration of $\tau > 0$ after each switch of the switching signal and then decrease exponentially at a rate of $\alpha$ till the next switch. We set $\alpha$ to zero and $\tau$ to $\infty$ to restrict the difference to be upper bounded by $\eps$ at all times with no requirement of exponential convergence. We consider the set of input signals to be $\Sigma(T_d)$ instead of $\mathcal{U}$ and $f_p(x)$ in (\ref{sys:switched_system}) to be equal to $f(x,p)$ in (\ref{sys:noise}). By doing this, the entropy definition in Section 2 in \cite{sibai-mitra-2017} would be identical to (\ref{def:entropy}). Then, using Theorem 1 in \cite{sibai-mitra-2017},  the entropy $h\est(\eps,K)$ of system~(\ref{sys:switched_system}) is upper bounded by:
  \begin{align}
  \label{eq:switched_switched_bound}
  \frac{nL_x}{\ln 2} + \frac{\log N}{T_e},
  \end{align}
   where $T_e \in (0,T_d]$ and is the largest positive real such that $d(T_e) \leq \eps$. 
   
   It is not obvious how to compare the two bounds. The bound (\ref{eq:input_switched_bound}) increases linearly with the number of modes $N$ while (\ref{eq:switched_switched_bound}) only scales logarithmically. $d(t)$ appears in (\ref{eq:input_switched_bound}) in the limit as part of $M_u$ definition while it appears explicitly evaluated at a particular time in (\ref{eq:switched_switched_bound}).  
 
 
 %However, the input signals that obey the constraints on the variation and only have values corresponding to the $[N]$ modes would have a minimum dwell time of $T_d$.
 
 
 
 
 
% If one knows a restriction on the switching such as switching based on neighborhood on a graph, she can design the map $g$ in a way where we can get a tighter bound on $\mu$ and $\eta$.
%Since in the bounds of Section~\ref{sec:main_upperbound} requires $\mu$ to be positive, we set it small enough such that $\rho(k,\delta_u)$ in Proposition~\ref{prop:specificUpperBound} is smaller than $\nicefrac{1}{M_x}$. 


==> upperBoundDiscussion.tex <==
\subsection{Entropy upper bound discussion}
\label{sec:main_upperbound_discussion}
In this section we discuss how the bound in Proposition~\ref{prop:specificUpperBound}
 %and Corollary~\ref{cor:better_nonlinear_upperbound} 
 changes with different system parameters. Remember that $\mu$ and $\jum$ bound the variation of the input signal and $u_{\mathit{max}}$ bounds its norm at any instant in time. %Specifically, we present how would the upper bound vary in four cases that result from the truth value of the two following statements: $b1$: the bound on the input $u_{\mathit{max}}$ is small relative to the estimation error $\varepsilon$, and $b_2$: the variation of the input signal represented by $\mu$ and $\eta$ relative to the estimation error $\varepsilon$. 
%
%Also, the second row represent the opposite case.
%\item As $\jum$ increases, $\rho(\nicefrac{1}{2},\jum)$ increases as well. This can be seen by differentiating $\rho(\nicefrac{1}{2},\jum)$ with respect to $\jum$ which results in: 
%\begin{align*}
%\frac{\partial \rho(\nicefrac{1}{2},\jum)}{\partial \jum} &=  \frac{2}{\mu}\bigg(-1 + \sqrt[3]{1 + \frac{c}{\jum^3}} - \frac{c}{\mu \jum \sqrt[3]{(\jum^3 + c)^{2}}}\bigg) \\
%&= \frac{2}{\mu}\bigg(-1 + \frac{1}{\jum}( \sqrt[3]{\jum^3 + c} - \frac{c}{\mu \sqrt[3]{(\jum^3 + c)^{2}}})\bigg),
%\end{align*}
%where $c =  \frac{3\mu}{8}\big(\frac{k_2\eps}{ M_u e^{M_x}}\big)^2$. It is positive for $\jum$ large enough. 
\begin{comment}The top left cell ($b_1 \ \wedge \ b_2$) corresponds to a negligible input, and  its impact on the state uncertainty (or equivalently the volume of the reach set) is also negligible. Unsurprisingly, we recover the upper bounds of Corollary~\ref{cor:relationToPrevBound}.
\item If ($b_1 \ \wedge \ \neg b_2$), the effect of the variation of the input signal is negligible with respect to the effect of the large norm. In this case, logarithm of the accuracy parameter $\varepsilon$  appears  along with $u_{\mathit{max}}$. This makes intuitive sense. Since entropy represents the exponential rate of increases in the number of distinguishable trajectories, we can conclude from this upper bound that inputs with large norm and small variation increase the number of distinguishable trajectories by at most a linear factor $(\frac{u_{\mathit{max}}M_u}{\eps M_x})^{mM_x}$.
\item If ($\neg b_1 \ \wedge \ b_2$)  the input depends only on the variation parameters and not on $u_{\mathit{max}}$ as what matters in this case is the high variation of the input instead of its norm. Remember that $\jum$ represents the maximum norm of a jump and $\mu$ roughly represents how often large jumps can happen in a short amount of time. For a fixed $\jum$, having a higher $\mu$ increases the upper bound by $\Omega(\sqrt{\mu})$, which is much larger than the effect of increasing $u_{\mathit{max}}$ in the previous bound, which was $\Omega(\log u_{\mathit{max}})$. This shows that variation of input have a more drastic effect on the state uncertainty of the system and at the rate we should collect information to estimate its state than its value. On the other hand, note that the term inside the $O(\cdot)$ is $\frac{n}{\Talgo}$ and for a fixed $\mu$, $\frac{\partial T_p}{\partial \jum} = \frac{-1}{\mu} + \frac{\nicefrac{\jum}{\mu}}{ \sqrt{\jum^2 + \nicefrac{2\eps \mu}{M_u3e}}}$ which is less than zero. Thus, having a larger $\jum$, increases the upper bound as expected. Additionally, the upper bound grows with $\Omega(\frac{1}{\sqrt{\eps}}$ while it was growing as $\log (\frac{1}{\eps})$ in the case of low variation and high values of inputs.
\end{comment}   
%Observe that the added term is linear in the variation parameters $\mu$ and $\jum$ in contrast with the logarithmic term added in the previous one. Hence, high variation of the input increase the number of distinguishable trajectories by at most an exponential term instead of linear one
\begin{enumerate}
\item The bound %in both the proposition and the corollary 
increases logarithmically in  $u_{\mathit{max}}$. 
%This means that the growth in the uncertainty in the state estimate because of the increase in the bound on the input is at least exponentially slower than the growth caused by its faster variation.
\item It increases linearly with $M_x$, state dimension $n$ and input dimension $m$.
\item It increases  
\item The entropy bound %in  Proposition~\ref{prop:specificUpperBound} and %Corollary~\ref{cor:better_nonlinear_upperbound} 
increases quadratically with $\jum$. That is expected as larger jumps in the input signal would lead to a higher uncertainty in the system's state.
\item As $\mu$ increases, 
%the bound in Corollary~\ref{cor:better_nonlinear_upperbound} will increase in the order of $\frac{1}{1 - O(\mu)}$ while 
the entropy bound % in Proposition~\ref{prop:specificUpperBound}
 increases as $O(\mu^{\nicefrac{2}{3}})$. %That is, if all the parameters are treated as constants. 
\item Finally, as $\eps$ goes to zero, the bound % in Proposition~\ref{prop:specificUpperBound}
 grows as $\Omega(\eps^{-\nicefrac{2}{3}})$.
% and that of Corollary~\ref{cor:better_nonlinear_upperbound} as $\Omega(\eps^{-2})$. 
\end{enumerate} 

